Single-sample versus case-control sampling scheme for Positive Unlabeled data: the story of two scenarios

In the paper we argue that performance of the classifiers based on Empirical Risk Minimization (ERM) for positive unlabeled data, which are designed for case-control sampling scheme may significantly deteriorate when applied to a single-sample scenario. We reveal why their behavior depends, in all but very specific cases, on the scenario. Also, we introduce a single-sample case analogue of the popular non-negative risk classifier designed for case-control data and compare its performance with the original proposal. We show that the significant differences occur between them, especiall when half or more positive of observations are labeled. The opposite case when ERM minimizer designed for the case-control case is applied for single-sample data is also considered and similar conclusions are drawn. Taking into account difference of scenarios requires a sole, but crucial, change in the definition of the Empirical Risk.

==> latex/CC-f1-p1.tex <==

\begin{tabular}{l|c|ccccccccc}
\toprule
	\textbf{c} & \textbf{Model} & \textbf{Beans} & \textbf{CIFAR} & \textbf{Chest X-ray} & \textbf{DogFood} & \textbf{EuroSAT} & \textbf{Fashion MNIST} & \textbf{MNIST} & \textbf{Oxford Pets} & \textbf{Snacks} \\
\midrule
	\multirow[c]{3}{*}{0.1} & nnPUss & 71.14 & 94.59 & 92.89 & 79.05 & 75.37 & 94.77 & 93.64 & 68.69 & 69.33 \\
	 & nnPUcc & 71.76 & 94.99 & 92.33 & 81.47 & 81.77 & 97.06 & 95.76 & 76.14 & 69.63 \\
	 & $\Delta$ & 0.62 & 0.41 & -0.57 & 2.41 & 6.40 & 2.29 & 2.12 & 7.45 & 0.30 \\
\midrule
	\multirow[c]{3}{*}{0.3} & nnPUss & 80.53 & 95.86 & 95.44 & 90.48 & 82.73 & 94.67 & 94.25 & 76.35 & 78.76 \\
	 & nnPUcc & 80.47 & 96.76 & 94.89 & 95.79 & 90.94 & 98.71 & 97.95 & 90.09 & 80.64 \\
	 & $\Delta$ & -0.06 & 0.90 & -0.55 & 5.31 & 8.21 & 4.03 & 3.70 & 13.73 & 1.87 \\
\midrule
	\multirow[c]{3}{*}{0.5} & nnPUss & 84.72 & 92.34 & 95.35 & 93.16 & 79.46 & 88.21 & 86.20 & 82.06 & 73.04 \\
	 & nnPUcc & 84.72 & 97.87 & 95.81 & 97.51 & 94.07 & 99.34 & 98.95 & 94.87 & 84.74 \\
	 & $\Delta$ & 0.00 & 5.53 & 0.46 & 4.35 & 14.61 & 11.13 & 12.75 & 12.81 & 11.70 \\
\midrule
	\multirow[c]{3}{*}{0.7} & nnPUss & 82.66 & 87.82 & 88.92 & 89.77 & 75.12 & 87.76 & 89.83 & 80.44 & 72.22 \\
	 & nnPUcc & 86.09 & 98.66 & 94.28 & 96.85 & 96.01 & 99.59 & 99.38 & 96.99 & 84.29 \\
	 & $\Delta$ & 3.42 & 10.84 & 5.36 & 7.08 & 20.89 & 11.83 & 9.55 & 16.56 & 12.07 \\
\midrule
	\multirow[c]{3}{*}{0.9} & nnPUss & 47.27 & 94.06 & 91.77 & 27.68 & 12.50 & 92.43 & 92.08 & 18.05 & 55.93 \\
	 & nnPUcc & 69.56 & 99.32 & 87.59 & 81.60 & 97.23 & 99.77 & 99.59 & 94.50 & 77.50 \\
	 & $\Delta$ & 22.29 & 5.26 & -4.18 & 53.91 & 84.74 & 7.33 & 7.51 & 76.45 & 21.57 \\
\bottomrule
\end{tabular}



==> latex/CC-f1-p2.tex <==

\begin{tabular}{l|c|ccccccccc}
\toprule
	\textbf{c} & \textbf{Model} & \textbf{California} & \textbf{Credit} & \textbf{Electricity} & \textbf{Wine} & \textbf{20News} & \textbf{HateSpeech} & \textbf{IMDB} & \textbf{PoemSentiment} & \textbf{SMSSpam} \\
\midrule
	\multirow[c]{3}{*}{0.1} & nnPUss & 82.45 & 66.44 & 74.32 & 69.11 & 82.00 & 0.00 & 72.41 & 7.38 & 36.99 \\
	 & nnPUcc & 82.81 & 67.37 & 75.04 & 71.25 & 83.44 & 0.00 & 73.75 & 5.31 & 30.33 \\
	 & $\Delta$ & 0.36 & 0.93 & 0.73 & 2.14 & 1.44 & 0.00 & 1.34 & -2.07 & -6.66 \\
\midrule
	\multirow[c]{3}{*}{0.3} & nnPUss & 85.54 & 71.56 & 78.13 & 71.83 & 83.71 & 34.42 & 71.84 & 44.10 & 80.68 \\
	 & nnPUcc & 87.03 & 73.10 & 78.95 & 77.06 & 87.64 & 38.94 & 78.21 & 41.61 & 86.37 \\
	 & $\Delta$ & 1.48 & 1.54 & 0.82 & 5.23 & 3.93 & 4.52 & 6.38 & -2.49 & 5.69 \\
\midrule
	\multirow[c]{3}{*}{0.5} & nnPUss & 87.39 & 76.16 & 81.21 & 76.63 & 78.87 & 32.08 & 74.80 & 55.17 & 79.65 \\
	 & nnPUcc & 89.26 & 77.83 & 81.75 & 81.65 & 90.34 & 49.95 & 80.95 & 59.11 & 92.79 \\
	 & $\Delta$ & 1.87 & 1.67 & 0.55 & 5.02 & 11.46 & 17.87 & 6.15 & 3.94 & 13.14 \\
\midrule
	\multirow[c]{3}{*}{0.7} & nnPUss & 90.07 & 80.34 & 83.89 & 79.64 & 80.82 & 6.47 & 78.05 & 45.80 & 47.23 \\
	 & nnPUcc & 91.68 & 82.49 & 84.54 & 85.44 & 93.01 & 56.17 & 84.07 & 66.88 & 94.47 \\
	 & $\Delta$ & 1.62 & 2.16 & 0.65 & 5.80 & 12.19 & 49.70 & 6.02 & 21.08 & 47.24 \\
\midrule
	\multirow[c]{3}{*}{0.9} & nnPUss & 89.91 & 82.10 & 85.19 & 81.38 & 89.11 & 0.00 & 81.48 & 0.00 & 0.78 \\
	 & nnPUcc & 94.24 & 85.59 & 87.69 & 90.05 & 96.11 & 53.40 & 87.81 & 54.04 & 90.68 \\
	 & $\Delta$ & 4.32 & 3.50 & 2.50 & 8.67 & 6.99 & 53.40 & 6.33 & 54.04 & 89.90 \\
\bottomrule
\end{tabular}



==> latex/CC-precision-p1.tex <==
\begin{tabular}{l|c|ccccccccc}
\toprule
	\textbf{c} & \textbf{Model} & \textbf{Beans} & \textbf{CIFAR} & \textbf{Chest X-ray} & \textbf{DogFood} & \textbf{EuroSAT} & \textbf{Fashion MNIST} & \textbf{MNIST} & \textbf{Oxford Pets} & \textbf{Snacks} \\
\midrule
	\multirow[c]{3}{*}{0.1} & nnPUss & 69.88 & 92.13 & 92.24 & 86.86 & 89.84 & 98.17 & 95.55 & 96.53 & 69.59 \\
	 & nnPUcc & 70.66 & 91.73 & 91.88 & 85.98 & 91.76 & 98.20 & 95.88 & 97.48 & 68.11 \\
	 & $\Delta$ & 0.78 & -0.40 & -0.36 & -0.88 & 1.92 & 0.03 & 0.33 & 0.95 & -1.49 \\
\midrule
	\multirow[c]{3}{*}{0.3} & nnPUss & 82.50 & 96.53 & 95.64 & 98.36 & 93.63 & 99.48 & 99.33 & 99.20 & 86.25 \\
	 & nnPUcc & 81.66 & 94.40 & 95.07 & 97.67 & 92.93 & 98.68 & 97.72 & 99.16 & 81.52 \\
	 & $\Delta$ & -0.85 & -2.13 & -0.57 & -0.69 & -0.70 & -0.80 & -1.61 & -0.04 & -4.73 \\
\midrule
	\multirow[c]{3}{*}{0.5} & nnPUss & 90.88 & 98.83 & 98.05 & 99.75 & 98.06 & 99.67 & 99.76 & 99.80 & 94.17 \\
	 & nnPUcc & 90.08 & 96.29 & 96.78 & 99.66 & 94.44 & 99.09 & 98.75 & 99.37 & 89.23 \\
	 & $\Delta$ & -0.80 & -2.55 & -1.27 & -0.09 & -3.62 & -0.58 & -1.01 & -0.43 & -4.95 \\
\midrule
	\multirow[c]{3}{*}{0.7} & nnPUss & 97.49 & 99.49 & 99.32 & 99.88 & 98.77 & 99.83 & 99.79 & 99.88 & 96.74 \\
	 & nnPUcc & 97.43 & 97.72 & 98.24 & 99.90 & 96.37 & 99.35 & 99.28 & 99.57 & 94.52 \\
	 & $\Delta$ & -0.07 & -1.77 & -1.08 & 0.01 & -2.40 & -0.48 & -0.51 & -0.31 & -2.22 \\
\midrule
	\multirow[c]{3}{*}{0.9} & nnPUss & 99.32 & 99.62 & 99.73 & 100.00 & 99.75 & 99.90 & 99.78 & 99.90 & 99.27 \\
	 & nnPUcc & 99.53 & 98.89 & 98.73 & 99.94 & 98.11 & 99.64 & 99.58 & 99.80 & 96.76 \\
	 & $\Delta$ & 0.21 & -0.73 & -1.00 & -0.06 & -1.64 & -0.26 & -0.20 & -0.10 & -2.51 \\
\bottomrule
\end{tabular}


==> latex/CC-precision-p2.tex <==

\begin{tabular}{l|c|ccccccccc}
\toprule
	\textbf{c} & \textbf{Model} & \textbf{California} & \textbf{Credit} & \textbf{Electricity} & \textbf{Wine} & \textbf{20News} & \textbf{HateSpeech} & \textbf{IMDB} & \textbf{PoemSentiment} & \textbf{SMSSpam} \\
\midrule
	\multirow[c]{3}{*}{0.1} & nnPUss & 81.21 & 65.61 & 79.28 & 71.19 & 81.08 & 0.00 & 76.76 & 23.75 & 99.00 \\
	 & nnPUcc & 80.02 & 65.02 & 78.31 & 70.97 & 81.05 & 0.00 & 75.83 & 20.00 & 89.57 \\
	 & $\Delta$ & -1.19 & -0.59 & -0.97 & -0.22 & -0.03 & 0.00 & -0.94 & -3.75 & -9.44 \\
\midrule
	\multirow[c]{3}{*}{0.3} & nnPUss & 89.47 & 74.41 & 85.39 & 80.97 & 87.17 & 61.88 & 85.07 & 79.24 & 96.27 \\
	 & nnPUcc & 86.19 & 72.45 & 85.09 & 79.43 & 85.56 & 59.57 & 82.71 & 81.66 & 94.78 \\
	 & $\Delta$ & -3.28 & -1.97 & -0.30 & -1.54 & -1.61 & -2.31 & -2.36 & 2.42 & -1.49 \\
\midrule
	\multirow[c]{3}{*}{0.5} & nnPUss & 92.21 & 80.09 & 89.20 & 87.65 & 91.12 & 77.01 & 88.95 & 85.26 & 99.33 \\
	 & nnPUcc & 89.87 & 78.57 & 88.69 & 85.61 & 89.27 & 67.95 & 87.32 & 79.83 & 96.68 \\
	 & $\Delta$ & -2.34 & -1.52 & -0.51 & -2.05 & -1.85 & -9.06 & -1.63 & -5.43 & -2.65 \\
\midrule
	\multirow[c]{3}{*}{0.7} & nnPUss & 94.79 & 86.07 & 93.06 & 91.36 & 94.63 & 92.39 & 92.60 & 95.10 & 99.92 \\
	 & nnPUcc & 93.35 & 85.22 & 92.84 & 90.30 & 93.06 & 77.90 & 91.67 & 90.85 & 98.21 \\
	 & $\Delta$ & -1.44 & -0.85 & -0.23 & -1.06 & -1.57 & -14.49 & -0.93 & -4.25 & -1.71 \\
\midrule
	\multirow[c]{3}{*}{0.9} & nnPUss & 98.03 & 94.78 & 97.28 & 95.87 & 97.32 & 0.00 & 96.92 & 0.00 & 20.00 \\
	 & nnPUcc & 97.14 & 94.65 & 97.05 & 95.61 & 96.68 & 91.34 & 96.68 & 96.93 & 99.30 \\
	 & $\Delta$ & -0.89 & -0.14 & -0.23 & -0.27 & -0.65 & 91.34 & -0.25 & 96.93 & 79.30 \\
\bottomrule
\end{tabular}



==> latex/CC-recall-p1.tex <==

\begin{tabular}{l|c|ccccccccc}
\toprule
	\textbf{c} & \textbf{Model} & \textbf{Beans} & \textbf{CIFAR} & \textbf{Chest X-ray} & \textbf{DogFood} & \textbf{EuroSAT} & \textbf{Fashion MNIST} & \textbf{MNIST} & \textbf{Oxford Pets} & \textbf{Snacks} \\
\midrule
	\multirow[c]{3}{*}{0.1} & nnPUss & 76.01 & 97.19 & 93.72 & 72.93 & 64.97 & 91.62 & 91.82 & 53.38 & 69.37 \\
	 & nnPUcc & 76.52 & 98.50 & 93.07 & 77.89 & 73.79 & 95.95 & 95.66 & 62.52 & 71.49 \\
	 & $\Delta$ & 0.51 & 1.31 & -0.66 & 4.96 & 8.82 & 4.34 & 3.84 & 9.14 & 2.12 \\
\midrule
	\multirow[c]{3}{*}{0.3} & nnPUss & 80.79 & 95.20 & 95.26 & 83.90 & 74.14 & 90.31 & 89.67 & 62.08 & 72.64 \\
	 & nnPUcc & 81.19 & 99.25 & 94.77 & 94.03 & 89.05 & 98.73 & 98.19 & 82.55 & 79.96 \\
	 & $\Delta$ & 0.39 & 4.05 & -0.49 & 10.13 & 14.91 & 8.42 & 8.52 & 20.47 & 7.32 \\
\midrule
	\multirow[c]{3}{*}{0.5} & nnPUss & 80.03 & 86.67 & 92.80 & 87.47 & 66.87 & 79.15 & 75.93 & 69.69 & 59.79 \\
	 & nnPUcc & 80.64 & 99.50 & 94.89 & 95.46 & 93.71 & 99.59 & 99.14 & 90.77 & 80.89 \\
	 & $\Delta$ & 0.61 & 12.83 & 2.09 & 7.99 & 26.84 & 20.44 & 23.21 & 21.07 & 21.09 \\
\midrule
	\multirow[c]{3}{*}{0.7} & nnPUss & 72.37 & 78.63 & 80.53 & 81.65 & 60.68 & 78.37 & 81.69 & 67.35 & 57.79 \\
	 & nnPUcc & 77.64 & 99.62 & 90.75 & 94.04 & 95.66 & 99.83 & 99.49 & 94.55 & 76.29 \\
	 & $\Delta$ & 5.27 & 20.99 & 10.22 & 12.39 & 34.98 & 21.47 & 17.79 & 27.20 & 18.50 \\
\midrule
	\multirow[c]{3}{*}{0.9} & nnPUss & 32.86 & 89.08 & 85.04 & 16.67 & 6.82 & 86.01 & 85.50 & 10.13 & 39.37 \\
	 & nnPUcc & 54.70 & 99.74 & 80.01 & 69.99 & 96.38 & 99.89 & 99.60 & 89.75 & 65.74 \\
	 & $\Delta$ & 21.84 & 10.66 & -5.03 & 53.32 & 89.56 & 13.88 & 14.10 & 79.62 & 26.36 \\
\bottomrule
\end{tabular}


==> latex/CC-recall-p2.tex <==
\begin{tabular}{l|c|ccccccccc}
\toprule
	\textbf{c} & \textbf{Model} & \textbf{California} & \textbf{Credit} & \textbf{Electricity} & \textbf{Wine} & \textbf{20News} & \textbf{HateSpeech} & \textbf{IMDB} & \textbf{PoemSentiment} & \textbf{SMSSpam} \\
\midrule
	\multirow[c]{3}{*}{0.1} & nnPUss & 83.83 & 67.44 & 69.97 & 67.29 & 82.96 & 0.00 & 68.53 & 4.50 & 23.99 \\
	 & nnPUcc & 85.88 & 70.00 & 72.06 & 71.65 & 86.00 & 0.00 & 71.79 & 3.07 & 19.58 \\
	 & $\Delta$ & 2.04 & 2.56 & 2.09 & 4.36 & 3.04 & 0.00 & 3.26 & -1.43 & -4.41 \\
\midrule
	\multirow[c]{3}{*}{0.3} & nnPUss & 82.02 & 69.58 & 72.06 & 64.66 & 80.53 & 23.98 & 62.18 & 31.69 & 69.52 \\
	 & nnPUcc & 87.90 & 74.33 & 73.68 & 74.93 & 89.84 & 28.99 & 74.19 & 28.83 & 79.56 \\
	 & $\Delta$ & 5.88 & 4.75 & 1.63 & 10.27 & 9.31 & 5.01 & 12.01 & -2.86 & 10.04 \\
\midrule
	\multirow[c]{3}{*}{0.5} & nnPUss & 83.11 & 73.08 & 74.57 & 68.23 & 69.55 & 20.36 & 64.54 & 41.72 & 66.54 \\
	 & nnPUcc & 88.74 & 77.74 & 75.86 & 78.10 & 91.44 & 39.72 & 75.45 & 48.24 & 89.34 \\
	 & $\Delta$ & 5.62 & 4.66 & 1.29 & 9.88 & 21.90 & 19.36 & 10.90 & 6.52 & 22.80 \\
\midrule
	\multirow[c]{3}{*}{0.7} & nnPUss & 85.81 & 75.85 & 76.38 & 70.70 & 70.55 & 3.37 & 67.46 & 30.95 & 31.44 \\
	 & nnPUcc & 90.09 & 80.35 & 77.62 & 81.14 & 92.97 & 44.07 & 77.64 & 53.67 & 91.07 \\
	 & $\Delta$ & 4.28 & 4.49 & 1.24 & 10.44 & 22.42 & 40.70 & 10.18 & 22.72 & 59.64 \\
\midrule
	\multirow[c]{3}{*}{0.9} & nnPUss & 83.08 & 72.50 & 75.81 & 70.92 & 82.19 & 0.00 & 70.29 & 0.00 & 0.40 \\
	 & nnPUcc & 91.51 & 78.18 & 79.99 & 85.18 & 95.54 & 37.88 & 80.44 & 38.80 & 83.50 \\
	 & $\Delta$ & 8.43 & 5.68 & 4.18 & 14.26 & 13.35 & 37.88 & 10.15 & 38.80 & 83.09 \\
\bottomrule
\end{tabular}


==> latex/SS-f1-p1.tex <==
\begin{tabular}{l|c|ccccccccc}
\toprule
	\textbf{c} & \textbf{Model} & \textbf{Beans} & \textbf{CIFAR} & \textbf{Chest X-ray} & \textbf{DogFood} & \textbf{EuroSAT} & \textbf{FashionMNIST} & \textbf{MNIST} & \textbf{Oxford Pets} & \textbf{Snacks} \\
\midrule
	\multirow[c]{3}{*}{0.1} & nnPUcc & 66.24 & 94.19 & 92.30 & 79.91 & 81.71 & 97.14 & 95.28 & 74.36 & 68.70 \\
	 & nnPUss & 61.48 & 93.20 & 92.80 & 76.76 & 76.04 & 94.99 & 93.71 & 65.67 & 67.93 \\
	 & $\Delta$ & -4.76 & -0.99 & 0.50 & -3.15 & -5.67 & -2.15 & -1.56 & -8.70 & -0.77 \\
\midrule
	\multirow[c]{3}{*}{0.3} & nnPUcc & 84.22 & 93.75 & 94.13 & 96.37 & 90.34 & 96.79 & 95.51 & 93.21 & 77.40 \\
	 & nnPUss & 82.71 & 94.97 & 94.95 & 92.60 & 85.15 & 96.96 & 96.80 & 81.24 & 77.20 \\
	 & $\Delta$ & -1.51 & 1.22 & 0.82 & -3.77 & -5.19 & 0.17 & 1.29 & -11.97 & -0.20 \\
\midrule
	\multirow[c]{3}{*}{0.5} & nnPUcc & 87.24 & 90.58 & 93.96 & 98.21 & 90.00 & 95.12 & 93.05 & 97.09 & 79.54 \\
	 & nnPUss & 87.65 & 95.96 & 95.41 & 97.18 & 90.01 & 97.98 & 98.26 & 88.85 & 81.74 \\
	 & $\Delta$ & 0.41 & 5.38 & 1.44 & -1.02 & 0.01 & 2.86 & 5.21 & -8.24 & 2.20 \\
\midrule
	\multirow[c]{3}{*}{0.7} & nnPUcc & 88.47 & 85.83 & 92.17 & 98.32 & 86.25 & 85.51 & 87.48 & 96.25 & 79.84 \\
	 & nnPUss & 91.31 & 97.10 & 95.84 & 99.01 & 92.65 & 99.11 & 99.00 & 93.77 & 84.47 \\
	 & $\Delta$ & 2.84 & 11.27 & 3.67 & 0.69 & 6.39 & 13.60 & 11.52 & -2.48 & 4.63 \\
\midrule
	\multirow[c]{3}{*}{0.9} & nnPUcc & 88.01 & 82.93 & 89.24 & 98.00 & 82.69 & 76.08 & 75.94 & 94.73 & 79.92 \\
	 & nnPUss & 93.49 & 97.99 & 96.57 & 99.71 & 94.83 & 99.44 & 99.21 & 98.35 & 86.89 \\
	 & $\Delta$ & 5.48 & 15.06 & 7.33 & 1.70 & 12.15 & 23.36 & 23.27 & 3.62 & 6.96 \\
\bottomrule
\end{tabular}


==> latex/SS-f1-p2.tex <==
\begin{tabular}{l|c|ccccccccc}
\toprule
	\textbf{c} & \textbf{Model} & \textbf{California} & \textbf{Credit} & \textbf{Electricity} & \textbf{Wine} & \textbf{20News} & \textbf{HateSpeech} & \textbf{IMDB} & \textbf{PoemSentiment} & \textbf{SMSSpam} \\
\midrule
	\multirow[c]{3}{*}{0.1} & nnPUcc & 82.43 & 67.12 & 74.80 & 69.65 & 82.96 & 0.00 & 73.01 & 1.18 & 20.45 \\
	 & nnPUss & 82.07 & 66.57 & 73.97 & 68.17 & 81.44 & 0.00 & 71.70 & 2.35 & 28.29 \\
	 & $\Delta$ & -0.36 & -0.54 & -0.83 & -1.48 & -1.52 & 0.00 & -1.31 & 1.18 & 7.84 \\
\midrule
	\multirow[c]{3}{*}{0.3} & nnPUcc & 84.39 & 70.78 & 78.62 & 75.52 & 85.70 & 29.84 & 77.50 & 11.54 & 85.11 \\
	 & nnPUss & 84.08 & 70.08 & 76.88 & 73.94 & 83.88 & 30.87 & 74.22 & 27.46 & 80.71 \\
	 & $\Delta$ & -0.31 & -0.70 & -1.74 & -1.58 & -1.82 & 1.03 & -3.28 & 15.92 & -4.40 \\
\midrule
	\multirow[c]{3}{*}{0.5} & nnPUcc & 84.37 & 70.99 & 80.48 & 78.44 & 85.64 & 42.47 & 79.36 & 29.54 & 91.42 \\
	 & nnPUss & 85.33 & 70.94 & 79.15 & 76.08 & 85.48 & 41.00 & 75.18 & 48.05 & 88.58 \\
	 & $\Delta$ & 0.95 & -0.05 & -1.34 & -2.36 & -0.16 & -1.47 & -4.18 & 18.51 & -2.84 \\
\midrule
	\multirow[c]{3}{*}{0.7} & nnPUcc & 82.93 & 71.02 & 80.58 & 79.47 & 83.94 & 47.28 & 79.57 & 52.70 & 93.89 \\
	 & nnPUss & 86.30 & 70.64 & 80.33 & 78.65 & 86.46 & 45.30 & 77.07 & 60.37 & 92.74 \\
	 & $\Delta$ & 3.38 & -0.38 & -0.25 & -0.81 & 2.51 & -1.98 & -2.50 & 7.67 & -1.15 \\
\midrule
	\multirow[c]{3}{*}{0.9} & nnPUcc & 80.82 & 70.81 & 79.23 & 79.11 & 81.19 & 49.51 & 78.55 & 59.71 & 94.85 \\
	 & nnPUss & 86.37 & 70.05 & 81.14 & 80.29 & 87.62 & 48.39 & 78.77 & 65.19 & 93.67 \\
	 & $\Delta$ & 5.55 & -0.76 & 1.91 & 1.18 & 6.43 & -1.11 & 0.22 & 5.48 & -1.18 \\
\bottomrule
\end{tabular}


==> latex/SS-precision-p1.tex <==
\begin{tabular}{l|c|ccccccccc}
\toprule
	\textbf{c} & \textbf{Model} & \textbf{Beans} & \textbf{CIFAR} & \textbf{Chest X-ray} & \textbf{DogFood} & \textbf{EuroSAT} & \textbf{FashionMNIST} & \textbf{MNIST} & \textbf{Oxford Pets} & \textbf{Snacks} \\
\midrule
	\multirow[c]{3}{*}{0.1} & nnPUcc & 82.98 & 90.11 & 90.88 & 89.28 & 92.74 & 97.62 & 94.47 & 99.59 & 70.35 \\
	 & nnPUss & 77.50 & 89.90 & 91.21 & 88.30 & 91.31 & 97.83 & 95.15 & 99.72 & 71.62 \\
	 & $\Delta$ & -5.48 & -0.20 & 0.33 & -0.98 & -1.44 & 0.20 & 0.68 & 0.13 & 1.27 \\
\midrule
	\multirow[c]{3}{*}{0.3} & nnPUcc & 86.94 & 88.41 & 91.84 & 97.43 & 89.56 & 93.79 & 91.53 & 99.53 & 74.45 \\
	 & nnPUss & 86.16 & 92.51 & 93.00 & 97.47 & 91.33 & 97.24 & 97.27 & 99.78 & 77.30 \\
	 & $\Delta$ & -0.77 & 4.09 & 1.17 & 0.04 & 1.78 & 3.45 & 5.74 & 0.26 & 2.85 \\
\midrule
	\multirow[c]{3}{*}{0.5} & nnPUcc & 83.14 & 82.81 & 91.72 & 97.77 & 83.92 & 90.71 & 87.04 & 97.68 & 73.93 \\
	 & nnPUss & 87.08 & 93.76 & 93.86 & 99.36 & 92.65 & 98.02 & 98.26 & 99.98 & 81.20 \\
	 & $\Delta$ & 3.93 & 10.95 & 2.14 & 1.59 & 8.73 & 7.31 & 11.22 & 2.30 & 7.27 \\
\midrule
	\multirow[c]{3}{*}{0.7} & nnPUcc & 81.97 & 75.18 & 91.03 & 97.42 & 76.65 & 74.76 & 77.80 & 93.87 & 72.64 \\
	 & nnPUss & 90.26 & 95.41 & 94.80 & 99.80 & 93.90 & 98.91 & 98.79 & 99.99 & 84.15 \\
	 & $\Delta$ & 8.29 & 20.23 & 3.76 & 2.38 & 17.25 & 24.14 & 20.99 & 6.13 & 11.51 \\
\midrule
	\multirow[c]{3}{*}{0.9} & nnPUcc & 81.71 & 70.85 & 90.14 & 96.64 & 70.86 & 61.39 & 61.23 & 90.34 & 71.83 \\
	 & nnPUss & 93.23 & 97.00 & 96.41 & 99.96 & 95.34 & 99.07 & 98.84 & 100.00 & 87.84 \\
	 & $\Delta$ & 11.52 & 26.14 & 6.27 & 3.32 & 24.48 & 37.68 & 37.62 & 9.66 & 16.01 \\
\bottomrule
\end{tabular}


==> latex/SS-precision-p2.tex <==
\begin{tabular}{l|c|ccccccccc}
\toprule
	\textbf{c} & \textbf{Model} & \textbf{California} & \textbf{Credit} & \textbf{Electricity} & \textbf{Wine} & \textbf{20News} & \textbf{HateSpeech} & \textbf{IMDB} & \textbf{PoemSentiment} & \textbf{SMSSpam} \\
\midrule
	\multirow[c]{3}{*}{0.1} & nnPUcc & 79.48 & 62.82 & 75.93 & 69.46 & 79.78 & 0.00 & 73.84 & 10.00 & 80.00 \\
	 & nnPUss & 80.85 & 63.22 & 76.93 & 69.72 & 79.86 & 0.00 & 74.69 & 20.00 & 99.77 \\
	 & $\Delta$ & 1.37 & 0.41 & 1.01 & 0.26 & 0.08 & 0.00 & 0.86 & 10.00 & 19.77 \\
\midrule
	\multirow[c]{3}{*}{0.3} & nnPUcc & 78.83 & 63.23 & 77.92 & 71.86 & 79.58 & 57.14 & 75.85 & 48.00 & 95.50 \\
	 & nnPUss & 84.06 & 65.97 & 81.01 & 75.10 & 82.08 & 55.47 & 78.96 & 55.04 & 92.94 \\
	 & $\Delta$ & 5.22 & 2.74 & 3.09 & 3.24 & 2.49 & -1.67 & 3.12 & 7.04 & -2.56 \\
\midrule
	\multirow[c]{3}{*}{0.5} & nnPUcc & 76.24 & 59.74 & 76.95 & 71.77 & 77.53 & 52.24 & 74.72 & 67.50 & 94.70 \\
	 & nnPUss & 85.29 & 62.80 & 81.15 & 76.70 & 83.88 & 52.74 & 80.96 & 70.25 & 92.48 \\
	 & $\Delta$ & 9.05 & 3.06 & 4.20 & 4.93 & 6.35 & 0.50 & 6.25 & 2.75 & -2.22 \\
\midrule
	\multirow[c]{3}{*}{0.7} & nnPUcc & 72.68 & 57.87 & 73.63 & 70.48 & 73.84 & 50.32 & 71.89 & 80.16 & 96.70 \\
	 & nnPUss & 86.10 & 59.65 & 81.76 & 77.79 & 84.96 & 53.35 & 81.58 & 76.51 & 93.85 \\
	 & $\Delta$ & 13.42 & 1.78 & 8.13 & 7.31 & 11.12 & 3.03 & 9.69 & -3.66 & -2.85 \\
\midrule
	\multirow[c]{3}{*}{0.9} & nnPUcc & 68.84 & 57.12 & 69.57 & 67.99 & 69.14 & 49.43 & 68.30 & 81.64 & 98.23 \\
	 & nnPUss & 86.20 & 56.81 & 81.42 & 78.09 & 86.02 & 53.92 & 81.01 & 80.15 & 92.39 \\
	 & $\Delta$ & 17.36 & -0.31 & 11.84 & 10.10 & 16.88 & 4.49 & 12.71 & -1.49 & -5.84 \\
\bottomrule
\end{tabular}


==> latex/SS-recall-p1.tex <==
\begin{tabular}{l|c|ccccccccc}
\toprule
	\textbf{c} & \textbf{Model} & \textbf{Beans} & \textbf{CIFAR} & \textbf{Chest X-ray} & \textbf{DogFood} & \textbf{EuroSAT} & \textbf{FashionMNIST} & \textbf{MNIST} & \textbf{Oxford Pets} & \textbf{Snacks} \\
\midrule
	\multirow[c]{3}{*}{0.1} & nnPUcc & 55.95 & 98.66 & 94.04 & 72.75 & 73.05 & 96.68 & 96.10 & 59.53 & 67.40 \\
	 & nnPUss & 51.67 & 96.76 & 94.62 & 68.51 & 65.20 & 92.33 & 92.33 & 49.28 & 64.81 \\
	 & $\Delta$ & -4.29 & -1.90 & 0.58 & -4.24 & -7.85 & -4.34 & -3.78 & -10.25 & -2.60 \\
\midrule
	\multirow[c]{3}{*}{0.3} & nnPUcc & 81.90 & 99.76 & 96.59 & 95.37 & 91.15 & 99.98 & 99.85 & 87.65 & 80.95 \\
	 & nnPUss & 79.76 & 97.57 & 97.01 & 88.24 & 79.77 & 96.68 & 96.33 & 68.59 & 77.22 \\
	 & $\Delta$ & -2.14 & -2.20 & 0.41 & -7.14 & -11.38 & -3.30 & -3.52 & -19.06 & -3.73 \\
\midrule
	\multirow[c]{3}{*}{0.5} & nnPUcc & 92.14 & 99.98 & 96.37 & 98.67 & 97.05 & 100.00 & 99.96 & 96.50 & 86.32 \\
	 & nnPUss & 88.57 & 98.28 & 97.01 & 95.14 & 87.52 & 97.95 & 98.26 & 79.97 & 82.39 \\
	 & $\Delta$ & -3.57 & -1.70 & 0.63 & -3.53 & -9.53 & -2.05 & -1.70 & -16.53 & -3.93 \\
\midrule
	\multirow[c]{3}{*}{0.7} & nnPUcc & 96.43 & 99.99 & 93.55 & 99.25 & 98.64 & 100.00 & 99.99 & 98.77 & 88.87 \\
	 & nnPUss & 92.62 & 98.85 & 96.91 & 98.24 & 91.44 & 99.31 & 99.21 & 88.28 & 84.83 \\
	 & $\Delta$ & -3.81 & -1.15 & 3.36 & -1.02 & -7.20 & -0.69 & -0.79 & -10.49 & -4.04 \\
\midrule
	\multirow[c]{3}{*}{0.9} & nnPUcc & 95.71 & 100.00 & 89.12 & 99.45 & 99.27 & 100.00 & 99.99 & 99.59 & 90.39 \\
	 & nnPUss & 93.81 & 99.01 & 96.74 & 99.45 & 94.33 & 99.81 & 99.57 & 96.76 & 85.98 \\
	 & $\Delta$ & -1.90 & -0.99 & 7.62 & 0.00 & -4.94 & -0.19 & -0.41 & -2.83 & -4.42 \\
\bottomrule
\end{tabular}


==> latex/SS-recall-p2.tex <==
\begin{tabular}{l|c|ccccccccc}
\toprule
	\textbf{c} & \textbf{Model} & \textbf{California} & \textbf{Credit} & \textbf{Electricity} & \textbf{Wine} & \textbf{20News} & \textbf{HateSpeech} & \textbf{IMDB} & \textbf{PoemSentiment} & \textbf{SMSSpam} \\
\midrule
	\multirow[c]{3}{*}{0.1} & nnPUcc & 85.77 & 72.17 & 73.73 & 69.90 & 86.41 & 0.00 & 72.20 & 0.62 & 12.46 \\
	 & nnPUss & 83.49 & 70.44 & 71.25 & 66.76 & 83.09 & 0.00 & 68.94 & 1.25 & 17.85 \\
	 & $\Delta$ & -2.29 & -1.74 & -2.48 & -3.14 & -3.32 & 0.00 & -3.26 & 0.62 & 5.40 \\
\midrule
	\multirow[c]{3}{*}{0.3} & nnPUcc & 90.86 & 80.52 & 79.37 & 79.66 & 92.84 & 20.29 & 79.23 & 6.88 & 76.89 \\
	 & nnPUss & 84.18 & 74.99 & 73.17 & 72.94 & 85.77 & 21.43 & 70.02 & 18.75 & 71.38 \\
	 & $\Delta$ & -6.68 & -5.54 & -6.20 & -6.72 & -7.08 & 1.15 & -9.22 & 11.88 & -5.51 \\
\midrule
	\multirow[c]{3}{*}{0.5} & nnPUcc & 94.57 & 87.65 & 84.36 & 86.53 & 95.64 & 35.82 & 84.63 & 19.38 & 88.45 \\
	 & nnPUss & 85.47 & 81.93 & 77.25 & 75.67 & 87.15 & 33.66 & 70.18 & 37.50 & 85.20 \\
	 & $\Delta$ & -9.10 & -5.72 & -7.11 & -10.86 & -8.50 & -2.16 & -14.46 & 18.13 & -3.25 \\
\midrule
	\multirow[c]{3}{*}{0.7} & nnPUcc & 96.62 & 92.10 & 89.00 & 91.11 & 97.25 & 44.67 & 89.08 & 40.00 & 91.31 \\
	 & nnPUss & 86.62 & 87.02 & 78.98 & 79.65 & 88.01 & 39.50 & 73.03 & 50.62 & 91.72 \\
	 & $\Delta$ & -10.00 & -5.08 & -10.03 & -11.46 & -9.24 & -5.17 & -16.05 & 10.62 & 0.41 \\
\midrule
	\multirow[c]{3}{*}{0.9} & nnPUcc & 97.89 & 93.27 & 92.00 & 94.60 & 98.34 & 49.67 & 92.42 & 48.12 & 91.71 \\
	 & nnPUss & 86.60 & 91.64 & 80.92 & 82.70 & 89.30 & 44.06 & 76.66 & 55.62 & 95.07 \\
	 & $\Delta$ & -11.29 & -1.62 & -11.07 & -11.90 & -9.04 & -5.61 & -15.76 & 7.50 & 3.37 \\
\bottomrule
\end{tabular}

